Synthetic Image Data for Deep Learning

Realistic synthetic image data rendered from 3D models can be used to augment image sets and train image classification semantic segmentation models. In this work, we explore how high quality physically-based rendering and domain randomization can efficiently create a large synthetic dataset based on production 3D CAD models of a real vehicle. We use this dataset to quantify the effectiveness of synthetic augmentation using U-net and Double-U-net models. We found that, for this domain, synthetic images were an effective technique for augmenting limited sets of real training data. We observed that models trained on purely synthetic images had a very low mean prediction IoU on real validation images. We also observed that adding even very small amounts of real images to a synthetic dataset greatly improved accuracy, and that models trained on datasets augmented with synthetic images were more accurate than those trained on real images alone. Finally, we found that in use cases that benefit from incremental training or model specialization, pretraining a base model on synthetic images provided a sizeable reduction in the training cost of transfer learning, allowing up to 90\% of the model training to be front-loaded.

==> sections/architecture.tex <==

%\subsubsection{Azure IoT Hub}
\begin{figure}[h!]
	  \centering
	  \includegraphics{ImportedFigures/architecture.jpeg}
	  \caption{{System Architecture Diagram}}
	  \label{fig:architecture}
	  %\vspace{-.1in}
\end{figure}

\begin{table}[!h]
\begin{center}
\caption{Iot Hub Editions and Throttling Limits}
\label{tab:throttle-limits}
\medskip
    \begin{tabular}{ccc}
    \hline\hline
    \noalign{\medskip}
    Edition & Max. D2C\textsuperscript{a} Send Operations & Max. Messages per Day\\
    \noalign{\medskip}
    \hline
    \noalign{\medskip}
    B1/S1 & 100 per sec\textsuperscript{b} & 400,000 per unit\\
    B2/S2  & 120 per sec per unit & 6,000,000 per unit\\
    B3/S3  & 6000 per sec per unit & 300,000,000 per unit\\
    \noalign{\medskip}
    \hline
    \noalign{\medskip}
    \multicolumn{3}{c}{Maximum Message Size is 256 KB}\\
    \noalign{\medskip}
    \hline\hline
    \noalign{\smallskip}
    \multicolumn{3}{l}{\textsuperscript{a}\footnotesize{Device-to-Cloud}}\\
    \multicolumn{3}{l}{\textsuperscript{b}\footnotesize{This is 12 per sec per unit if it results in a higher value.}}\\
    \end{tabular}
\end{center}
\end{table}

